A Robust and Constrained Multi-Agent Reinforcement Learning Electric Vehicle Rebalancing Method in AMoD Systems

Electric vehicles (EVs) play critical roles in autonomous mobility-on-demand (AMoD) systems, but their unique charging patterns increase the model uncertainties in AMoD systems (e.g. state transition probability). Since there usually exists a mismatch between the training and test/true environments, incorporating model uncertainty into system design is of critical importance in real-world applications. However, model uncertainties have not been considered explicitly in EV AMoD system rebalancing by existing literature yet, and the coexistence of model uncertainties and constraints that the decision should satisfy makes the problem even more challenging. In this work, we design a robust and constrained multi-agent reinforcement learning (MARL) framework with state transition kernel uncertainty for EV AMoD systems. We then propose a robust and constrained MARL algorithm (ROCOMA) with robust natural policy gradients (RNPG) that trains a robust EV rebalancing policy to balance the supply-demand ratio and the charging utilization rate across the city under model uncertainty. Experiments show that the ROCOMA can learn an effective and robust rebalancing policy. It outperforms non-robust MARL methods in the presence of model uncertainties. It increases the system fairness by 19.6% and decreases the rebalancing costs by 75.8%.

==> 003_sec_background.tex <==
In this section, we introduce the notation and theoretical foundations underlying our work in the context of Multi-Agent Reinforcement Learning (Subsection \ref{subsec_marl}) and robust and constrained Multi-Agent Reinforcement Learning (Subsection \ref{subsec_rocomarl}).

\subsection{Multi-Agent Reinforcement Learning Problem}
\label{subsec_marl}

We denote a Multi-Agent Reinforcement Learning (MARL) problem with a tuple $G = <\mathcal{N}, S, A, r,p,\gamma>$, in which $\mathcal{N}$ is the set of $N$ agents. Each agent is associated with an action $a^i \in A^i$ and a state $s^i \in S$. We use $A = A^1 \times \cdots \times A^N$ to denote the joint action space, and $S = S^1 \times \cdots \times S^N$  the joint state space. At time $t$, each agent chooses an action $a^i_t$ according to a policy $\pi^i: S^i \rightarrow \Delta(A^i)$, where $\Delta(A^i)$ represents the set of probability distributions over the action set $A^i$. We use $\pi = \prod_i^N \pi^i: S \rightarrow \Delta(A)$ to denote the joint policy. After executing the joint action, the next state follows the state transition probability which depends on the current state and the joint action, i.e.  $p: S \times A \rightarrow \Delta(S)$. And each agent receive a reward according to the reward function $r^i: S \times A \rightarrow \mathbb{R}$. Each agent aims to learn a policy $\pi^i$ to maximize its expected total discounted reward, i.e. $\max_{\pi^i} v^{\pi, i}_r(s)$ for all $s \in S$, where $v^{\pi, i}_r(s) = \mathbb{E}[\sum_{t = 1}^{\infty} \gamma^{t-1} r_t^i(s_t, a_t) | a_t \sim \pi(\cdot | s_t), s_1 = s]$ which is also known as the state value function for agent $i$. $\gamma \in (0,1]$ is the discounted rate. If these agents belong to a team, the objective of all agents is to collaboratively maximize the average expected total discounted reward over all agents, i.e. $\max_\pi v^{\pi}_{r}(s)$ for all $s \in S$, where $v^{\pi}_{r}(s) = \mathbb{E}[\sum_{t = 1}^{\infty} \gamma^{t-1} \bar{r}(s_t, a_t) | a_t \sim \pi(\cdot | s_t), s_1 = s]$, $\bar{r}(s_t, a_t) = N^{-1} \sum_{i\in \mathcal{N}}r_t^i(s_t, a_t)$.

\subsection{Robust and Constrained MARL}
\label{subsec_rocomarl}
In a robust and constrained Multi-Agent Reinforcement Learning problem, we consider the transition kernel $p$ is contained in a transition kernel uncertainty set $P$. And in this paper, we consider a team setting. We define the worst-case value function of a joint policy $\pi$ as the worst-case expected total discounted team reward following joint policy $\pi$ over the transition kernel uncertainty set:
\begin{align}
    v^\pi_r(s) = \min_{p \in P} \mathbb{E}\left[ \sum_{t=1}^\infty \gamma^{t-1}\bar{r}_t | a_t \sim \pi(\cdot|s_t), s_1 = s \right]
\end{align}
We then argument the MARL problem $G$ with a set $C$ of auxiliary cost functions, $c_1, \cdots, c_m$, and limits $d_1, \cdots, d_m$. Each function $c_i: S \times A  \rightarrow \mathbb{R}$ mapping transition tuples to costs, like the usual reward. Similarly, we let $v^{\pi, i}_c(s)$ denote the worst-case state value function of policy $\pi$ with respect to cost function $c_i$: $v^{\pi, i}_c(s) = \max_{p \in P}\mathbb{E} [\sum_{t=1}^{\infty} \gamma^{t-1} c_{i}(s_{t}, a_{t}) | a_{t} \sim \pi(\cdot | s_{t}), s_1 = s]$. The set of feasible policies for a roco MARL is then $\Pi_{C} := \{ \pi : \forall i, s\in S, v^{\pi, i}_c(s) \leq d_i \}$. We consider parameterized policies, i.e. $\pi(\cdot | \theta)$. 

The goal of a robust and constrained MARL is to find an optimal joint policy $\pi^*$ such that maximizes the worst-case value function subject to constraints on the expected utility for all $s \in S$: $\pi^* = \argmax_{\pi \in \Pi_{C}} v^{\pi}_r(s)$.
It is equivalent to the following max-min problem:
$$\max_{\theta} \min_{\lambda_i \geq 0} J(\theta, \lambda) := v^{\pi_\theta}_r(s) - \sum_{i=1}^m \lambda_i (v^{\pi_\theta,i}_c(s) - d_i)$$
It can be solved by Gradient Descent Ascent (GDA)~\cite{lin2020gradient} which currently is a widely-used algorithm for solving minimax optimization problems. At each iteration, GDA simultaneously performs gradient descent update on the variable $\lambda$ and gradient ascent update on the variable $\theta$ according to \eqref{def_robust_gda} with step sizes $\alpha_t$ and $\beta_{t}$.
\begin{align}
    \theta_{t+1} = \theta_t + \alpha_t (\nabla_\pi v^{\pi}_r(s)  - \lambda\nabla_\pi v^{\pi}_c(s))
    \nonumber \\
    \lambda_{i,t+1} = \lambda_{i,t} - \beta_{i,t} ( d_i - v^{\pi,i}_c(s) - \chi_{i,t} \lambda_{i,t})
    \label{def_robust_gda}
\end{align}




